A Unified BEV Model for Joint Learning of 3D Local Features and Overlap Estimation

Pairwise point cloud registration is a critical task for many applications, which heavily depends on finding correct correspondences from the two point clouds. However, the low overlap between input point clouds causes the registration to fail easily, leading to mistaken overlapping and mismatched correspondences, especially in scenes where non-overlapping regions contain similar structures. In this paper, we present a unified bird's-eye view (BEV) model for jointly learning of 3D local features and overlap estimation to fulfill pairwise registration and loop closure. Feature description is performed by a sparse UNet-like network based on BEV representation, and 3D keypoints are extracted by a detection head for 2D locations, and a regression head for heights. For overlap detection, a cross-attention module is applied for interacting contextual information of input point clouds, followed by a classification head to estimate the overlapping region. We evaluate our unified model extensively on the KITTI dataset and Apollo-SouthBay dataset. The experiments demonstrate that our method significantly outperforms existing methods on overlap estimation, especially in scenes with small overlaps. It also achieves top registration performance on both datasets in terms of translation and rotation errors.

==> BCLOUD <==
#edit-mode: -*- python -*-
#coding:utf-8

#相关帮助链接:
#    1. bcloud使用手册        : http://buildcloud.baidu.com/bcloud
#    2. bcloud各标签说明和用法: http://buildcloud.baidu.com/bcloud/6-bcloud_syntax
#    3. bcloud常见FAQ         : http://buildcloud.baidu.com/bcloud_faq

WORKROOT('../../../')

#platform, if not write PLATFORM('xxx') in BCLOUD file, default is 'centos4u3'
#PLATFORM('centos4u3')

#gcc version
GCC('gcc82')

#Preprocessor flags.
#CPPFLAGS(r'-D_GNU_SOURCE -D__STDC_LIMIT_MACROS')
#CPPFLAGS(r'-DVERSION=\"%s\"' % REPO_REVISION())

#C flags.
#global_cflags_str='-g -pipe -W -Wall -fPIC'
#CFLAGS(global_cflags_str)

#C++ flags.
#global_cxxflags_str='-g -pipe -W -Wall -fPIC'
#CXXFLAGS(global_cxxflags_str)

#-I path
#INCPATHS('. ./include $INC')

#libs which need to link with
#LIBS('$OUT/lib/libbev-overlap-feat_1.a')
#LIBS('$OUT/lib/libbev-overlap-feat_3.so')

#link flags
#LDFLAGS('-lpthread -lrt')

#CONFIGS("baidu/bcloud-demo/hello-svn@stable")

#user_sources=GLOB("*.c *.cpp *.cc *.proto")

#release headers
#HEADERS('*.h', '$INC')
#HEADERS('*.hpp', '$INC')
#HEADERS('include/*.h', '$INC')
#HEADERS('include/*.hpp', '$INC')

#release files except headers
#OUTPUT('conf', '$OUT')

#bin
#Notice:
#    1. CppFlags、CFlags、CxxFlags是Sources标签的参数
#    2. 局部标签CppFlags、CFlags、CxxFlags、LdFlags指定的参数会覆盖全局标签CPPFLAGS、CFLAGS、CXXFLAGS、LDFLAGS指定的参数，即局部覆盖全局
#Application('bev-overlap-feat',
#             Sources(user_sources,
#                     CppFlags('-DDEBUG'),
#                     CFlags('global_cxxflags_str' + ' -O3'),
#                     CxxFlags(global_cxxflags_str + ' -O3')),
#             LdFlags('-lpthread'))

#UT
#UTApplication('bev-overlap-feat_test',
#               Sources(user_sources),
#               UTOnServer(True))

#.a
#StaticLibrary('bev-overlap-feat_1',
#               Sources(user_sources))

#发布已经编译好的静态库，该用法要求libbev-overlap-feat_2.a文件必须位于代码根目录中的lib子目录下
#StaticLibrary('bev-overlap-feat_2',
#               PreBuilt(True))

#.so
#SharedLibrary('bev-overlap-feat_3',
#               Sources(user_sources))

#发布已经编译好的动态库，该用法要求libbev-overlap-feat4.so文件必须位于代码根目录中的lib子目录下
#SharedLibrary('bev-overlap-feat_4',
#               PreBuilt(True))

#sub directory
#Directory('demo')


